Improving Node Representation by Boosting Target-Aware Contrastive Loss

Graphs model complex relationships between entities, with nodes and edges capturing intricate connections. Node representation learning involves transforming nodes into low-dimensional embeddings. These embeddings are typically used as features for downstream tasks. Therefore, their quality has a significant impact on task performance. Existing approaches for node representation learning span (semi-)supervised, unsupervised, and self-supervised paradigms. In graph domains, (semi-)supervised learning often only optimizes models based on class labels, neglecting other abundant graph signals, which limits generalization. While self-supervised or unsupervised learning produces representations that better capture underlying graph signals, the usefulness of these captured signals for downstream target tasks can vary. To bridge this gap, we introduce Target-Aware Contrastive Learning (Target-aware CL) which aims to enhance target task performance by maximizing the mutual information between the target task and node representations with a self-supervised learning process. This is achieved through a sampling function, XGBoost Sampler (XGSampler), to sample proper positive examples for the proposed Target-Aware Contrastive Loss (XTCL). By minimizing XTCL, Target-aware CL increases the mutual information between the target task and node representations, such that model generalization is improved. Additionally, XGSampler enhances the interpretability of each signal by showing the weights for sampling the proper positive examples. We show experimentally that XTCL significantly improves the performance on two target tasks: node classification and link prediction tasks, compared to state-of-the-art models.

==> fig/order_algo.tex <==
\begin{algorithm}[t]
\caption{Training Order Determination}\label{alg:eval_order}
\begin{algorithmic}[1]
\REQUIRE {\rt}s $\{f_{r, u}|r\in\sR, u\in U_{L}\}$, semantic relations $\sR$, training instance $U_{L}$
\ENSURE $\overline{\sR}=\{r_1, r_2, \cdots, r_{|\sR|}\}$
\FORALL{$r\in\sR$}
    \FORALL{$u\in U_L$}
        \STATE $\widehat{p}(f_{r,u}|\sI_t)\gets\frac{\vert\{v|f_{r,u}(v)=1, \sI_t(u,v)=1), v\in U_L\}\vert}{\vert\{v|\sI_t(u,v)=1), v\in U_L\}\vert}$ 
        \STATE $\widehat{p}(\sI_t)\gets\frac{\vert\{v| \sI_t(u,v)=1), v\in U_L\}\vert}{\vert U_L\vert}$
        \STATE $\widehat{p}(f_{r,u})\gets\frac{\vert\{v|f_{r,u}(v)=1, v\in\gV\}\vert}{\vert \gV \vert}$ 
        \STATE $\widetilde{\sP}_u\gets\frac{\widehat{p}(f_{r,u}|\sI_t)\widehat{p}(\sI_t)}{\widehat{p}(f_{r,u})}$ 
    \ENDFOR
    \STATE $\widetilde{\sP}_r \gets \frac{1}{|V_q|}\widetilde{\sP}_u$
\ENDFOR
\STATE $\overline{\sR}\gets$sort $r\in\sR$ in $\widetilde{\sP}_r$ descending order
\end{algorithmic}
\end{algorithm}

==> fig/overfitting.tex <==


\begin{figure}[t]
\centering
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=\linewidth]{fig/acc_diff_label_attr_dist.pdf}
  \caption{Attribute Dist. Similarity.}
  \label{fig:acc_diff_attr_dist}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=\linewidth]{fig/acc_diff_topology.pdf}
  \caption{Topology Similarity.}
  \label{fig:acc_diff_topology}
\end{subfigure}
\vspace{-7mm}
\caption{This figure shows the severity of overfitting among different models. The severity is quantified by the accuracy difference between training and testing (training accuracy - testing accuracy).}
\label{fig:overfitting}
\vspace{-1mm}
\end{figure}

==> fig/perturb_fig.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=\linewidth]{fig/perturb_label_attr_dist.pdf}
  \caption{Node Classification ACC.}
  \label{fig:perturb_attr_dist}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=\linewidth]{fig/acc_diff_label_attr_dist.pdf}
  \caption{Train ACC - Test ACC.}
  \label{fig:acc_diff_attr_dist}
\end{subfigure}
\vspace{-4mm}
\caption{Results on semi-synthetic data when varying the dependency between node labels and a graph signal (1-Hop Attr. Dist.). The results show that minimizing losses, which are not task-aware, is {\em not} equivalent to maximizing the mutual information $\gI(\mY;Z)$, which decreases model generalization on node classification.}
\label{fig:motivation_exp}
\vspace{-4mm}
\end{figure}

==> fig/sup_vs_out.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/sup_vs_our.pdf}
  \vspace{-7mm}
  \caption{Learning curves of GCN trained with various supervision signals. Our {\xgs} is effective because {\loss} continues to outperform others when the training size increases.}
  \vspace{-4mm}
  \label{fig:sup_vs_our}
\end{figure}

==> fig/time_cost.tex <==
\begin{table}[t]
\caption{Computational Time in seconds.}
\vspace{-4mm}
\setlength{\tabcolsep}{2pt}
\label{tab:time}
\begin{center}
\begin{tabular}{lrrrrr}
\hline
 & Cora & CiteSeer & PubMed & Photo & Computers \\
\hline
XGBoost & 4.05 & 4.89 & 66.19 & 17.76 & 41.81 \\
{\xgs} & 0.77 & 0.9 & 10.59 & 2.31 & 5.65 \\
GCN Training & 4.15 & 5.95 & 40.79 & 31.33 & 34.40 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> fig/xgboost_algo.tex <==
\begin{algorithm}[t]
\caption{XGBoost Sampler Training}\label{alg:xgboost}
\begin{algorithmic}[1]
\REQUIRE Ordered semantic relation set $\overline{\sR}=\{r_1, r_2, \cdots, r_{|\sR|}\}$, training instances $U_{L}$
\ENSURE Classifiers ${f_u|u\in\gV}$
\STATE Initialize all $\hat{y}^{(0)}_{u,v}=0$
\FORALL{$i\in \{1,2,\cdots, |\sR|\}$}
    \FORALL{$(u,v)\in U_{L}\times U_{L}$}
        \STATE $g_{u,v}\gets \sigma(\hat{y}^{(i-1)}_{u,v})-y_{u,v}$
        \STATE $h_{u,v}\gets \sigma(\hat{y}^{(i-1)}_{u,v})(1-\sigma(\hat{y}^{(i-1)}_{u,v}))$
    \ENDFOR
    \STATE $w_{r_i,0}\gets\eqref{eq:w0}$
    \STATE $w_{r_i,1}\gets\eqref{eq:w1}$
    \FORALL{$(u,v)\in U_{L}\times U_{L}$}
        \IF{$s_{r_i}(u,v)>\eta_{r_i, u}$}
            \STATE $\hat{y}^{(i)}_{u,v}=\hat{y}^{(i-1)}_{u,v}+w_{r_i,1}$
        \ELSE
            \STATE $\hat{y}^{(i)}_{u,v}=\hat{y}^{(i-1)}_{u,v}+w_{r_i,0}$
        \ENDIF
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}


